Pred-NBV: Prediction-guided Next-Best-View for 3D Object Reconstruction

Prediction-based active perception has shown the potential to improve the navigation efficiency and safety of the robot by anticipating the uncertainty in the unknown environment. The existing works for 3D shape prediction make an implicit assumption about the partial observations and therefore cannot be used for real-world planning and do not consider the control effort for next-best-view planning. We present Pred-NBV, a realistic object shape reconstruction method consisting of PoinTr-C, an enhanced 3D prediction model trained on the ShapeNet dataset, and an information and control effort-based next-best-view method to address these issues. Pred-NBV shows an improvement of 25.46% in object coverage over the traditional methods in the AirSim simulator, and performs better shape completion than PoinTr, the state-of-the-art shape completion model, even on real data obtained from a Velodyne 3D LiDAR mounted on DJI M600 Pro.

==> tables/all_models_respective.tex <==
% https://tex.stackexchange.com/questions/156219/proper-centering-with-cmidrule-and-multi-row-and-column
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
% \begin{tabular}{ld{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}d{3.3}}
\toprule
\multirow{2}[3]{*}{Model Name} & \multicolumn{3}{c}{Baseline (R:$0^\circ$, T:0)} & \multicolumn{3}{c}{Ours (R: $25^\circ$, T: 0)} & \multicolumn{3}{c}{Ours (R: $25^\circ$, T: 0.1)} & \multicolumn{3}{c}{Ours (R: $45^\circ$, T: 0.1)} & \multicolumn{3}{c}{Ours (R: $45^\circ$, T: 0.25)} & \multicolumn{3}{c}{Ours (R: $90^\circ$, T: 0.25)} & \multicolumn{3}{c}{Ours (R: $90^\circ$, T: 0.5)} & \multicolumn{3}{c}{Ours (R: $180^\circ$, T: 0.5)} & \multicolumn{3}{c}{Ours (R: $360^\circ$, T: 0.5)} \\
% \midrule
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13}  \cmidrule(lr){14-16}  \cmidrule(lr){17-19}  \cmidrule(lr){20-22}  \cmidrule(lr){23-25} \cmidrule(lr){26-28} 
{}  &             F-Score &    CDL1 &   CDL2 &            F-Score &    CDL1 &    CDL2 &              F-Score &    CDL1 &    CDL2 &              F-Score &    CDL1 &    CDL2 &               F-Score &    CDL1 &    CDL2 &               F-Score &    CDL1 &    CDL2 &              F-Score &    CDL1 &    CDL2 &               F-Score &    CDL1 &    CDL2 &               F-Score &    CDL1 &    CDL2 \\
% Model Name  &                     &         &        &                    &         &         &                      &         &         &                      &         &         &                       &         &         &                       &         &         &                      &         &         &                       &         &         &                       &         &         \\

\midrule
microphone  &               0.663 &   9.916 &  0.699 &              0.631 &  19.876 &   6.732 &                0.704 &  20.077 &   7.271 &                0.702 &  20.928 &   7.854 &                 0.715 &  24.763 &  11.391 &                 0.697 &  28.295 &  14.333 &                0.715 &  37.941 &  28.814 &                 0.726 &  34.210 &  26.889 &                 0.725 &  34.434 &  29.081 \\
stove       &               0.426 &  12.744 &  0.628 &              0.444 &  31.492 &  15.931 &                0.521 &  30.239 &  17.307 &                0.512 &  29.905 &  15.831 &                 0.530 &  32.611 &  20.117 &                 0.526 &  34.107 &  21.168 &                0.539 &  45.759 &  37.122 &                 0.541 &  43.722 &  34.472 &                 0.545 &  43.602 &  36.000 \\
earphone    &               0.449 &  13.492 &  0.812 &              0.445 &  17.639 &   3.283 &                0.540 &  19.435 &   5.350 &                0.524 &  21.576 &   6.282 &                 0.560 &  28.667 &  13.019 &                 0.556 &  29.995 &  14.313 &                0.581 &  44.597 &  37.056 &                 0.582 &  42.063 &  31.383 &                 0.589 &  39.620 &  28.464 \\
helmet      &               0.365 &  15.451 &  0.989 &              0.357 &  23.051 &   5.350 &                0.452 &  24.310 &   7.949 &                0.444 &  26.828 &   9.754 &                 0.479 &  35.526 &  19.604 &                 0.478 &  36.940 &  20.848 &                0.509 &  51.349 &  41.359 &                 0.512 &  49.150 &  38.449 &                 0.514 &  48.334 &  39.469 \\
tower       &               0.549 &  11.172 &  0.548 &              0.549 &  22.278 &   7.744 &                0.612 &  22.677 &   9.195 &                0.608 &  23.229 &   9.350 &                 0.619 &  29.829 &  16.582 &                 0.615 &  31.612 &  18.772 &                0.627 &  46.606 &  41.516 &                 0.636 &  41.206 &  34.379 &                 0.642 &  41.147 &  37.263 \\
train       &               0.519 &  10.768 &  0.502 &              0.499 &  18.138 &   4.232 &                0.554 &  19.800 &   6.010 &                0.543 &  22.396 &   6.981 &                 0.565 &  31.132 &  16.889 &                 0.557 &  33.632 &  19.024 &                0.602 &  45.224 &  40.279 &                 0.600 &  43.613 &  39.422 &                 0.610 &  42.028 &  38.957 \\
microwaves  &               0.385 &  13.671 &  0.670 &              0.413 &  44.618 &  28.869 &                0.492 &  41.156 &  27.348 &                0.478 &  40.319 &  26.065 &                 0.510 &  41.447 &  29.498 &                 0.507 &  42.166 &  30.388 &                0.526 &  46.961 &  38.837 &                 0.528 &  46.193 &  36.262 &                 0.525 &  46.741 &  39.347 \\
printer     &               0.409 &  13.415 &  0.734 &              0.416 &  30.601 &  12.730 &                0.497 &  27.563 &  12.394 &                0.488 &  27.793 &  11.866 &                 0.509 &  30.729 &  17.032 &                 0.506 &  32.724 &  18.598 &                0.527 &  43.124 &  33.371 &                 0.532 &  43.954 &  33.826 &                 0.537 &  42.179 &  31.680 \\
pillow      &               0.425 &  12.565 &  0.610 &              0.428 &  13.710 &   1.208 &                0.510 &  16.000 &   3.389 &                0.503 &  17.371 &   3.971 &                 0.533 &  27.507 &  14.936 &                 0.530 &  28.532 &  15.588 &                0.570 &  40.643 &  34.230 &                 0.572 &  40.373 &  32.655 &                 0.572 &  39.725 &  33.412 \\
cellphone   &               0.542 &   9.515 &  0.321 &              0.507 &  20.226 &   6.360 &                0.575 &  20.980 &   7.910 &                0.562 &  21.179 &   7.206 &                 0.570 &  28.946 &  15.216 &                 0.564 &  29.751 &  15.821 &                0.586 &  45.535 &  38.399 &                 0.590 &  47.679 &  42.926 &                 0.598 &  43.722 &  38.341 \\
bathtub     &               0.430 &  12.699 &  0.642 &              0.429 &  21.281 &   5.970 &                0.501 &  22.000 &   7.708 &                0.492 &  22.110 &   7.342 &                 0.518 &  28.839 &  14.432 &                 0.515 &  30.468 &  15.751 &                0.547 &  40.885 &  30.172 &                 0.551 &  39.767 &  28.461 &                 0.552 &  39.785 &  30.022 \\
watercraft  &               0.606 &   9.359 &  0.413 &              0.590 &  18.230 &   4.669 &                0.637 &  19.610 &   6.649 &                0.625 &  22.021 &   7.574 &                 0.637 &  29.666 &  16.174 &                 0.623 &  34.034 &  21.190 &                0.651 &  47.429 &  45.334 &                 0.663 &  40.480 &  36.094 &                 0.666 &  38.979 &  34.600 \\
bookshelf   &               0.398 &  13.421 &  0.711 &              0.400 &  21.933 &   7.296 &                0.486 &  21.255 &   7.769 &                0.477 &  22.561 &   7.811 &                 0.496 &  31.215 &  16.663 &                 0.494 &  32.256 &  16.992 &                0.519 &  46.621 &  36.757 &                 0.523 &  45.490 &  34.487 &                 0.524 &  45.120 &  36.040 \\
jar         &               0.416 &  13.706 &  0.772 &              0.422 &  20.701 &   5.225 &                0.497 &  20.755 &   6.242 &                0.488 &  21.915 &   6.632 &                 0.512 &  28.488 &  13.090 &                 0.510 &  29.609 &  13.964 &                0.533 &  47.355 &  38.203 &                 0.537 &  43.768 &  33.467 &                 0.542 &  42.144 &  33.042 \\
washer      &               0.375 &  14.231 &  0.745 &              0.411 &  37.926 &  22.758 &                0.490 &  36.989 &  23.603 &                0.480 &  37.528 &  22.842 &                 0.502 &  39.109 &  27.096 &                 0.502 &  38.926 &  26.231 &                0.518 &  46.540 &  37.752 &                 0.521 &  45.058 &  35.580 &                 0.519 &  45.971 &  38.084 \\
guitar      &               0.875 &   5.616 &  0.145 &              0.697 &  15.582 &   3.826 &                0.756 &  20.082 &   6.516 &                0.760 &  18.538 &   5.857 &                 0.761 &  27.481 &  14.194 &                 0.756 &  27.529 &  13.989 &                0.745 &  45.950 &  41.859 &                 0.761 &  39.648 &  34.128 &                 0.776 &  37.818 &  34.205 \\
telephone   &               0.548 &   9.403 &  0.314 &              0.503 &  19.543 &   5.969 &                0.577 &  21.485 &   8.302 &                0.564 &  21.374 &   7.469 &                 0.576 &  29.911 &  16.347 &                 0.567 &  31.115 &  17.578 &                0.594 &  47.336 &  41.487 &                 0.601 &  47.090 &  41.580 &                 0.607 &  45.154 &  41.228 \\
cap         &               0.427 &  11.647 &  0.458 &              0.459 &  17.737 &   3.610 &                0.535 &  20.816 &   7.230 &                0.521 &  23.424 &   8.361 &                 0.551 &  33.220 &  18.782 &                 0.545 &  33.683 &  19.614 &                0.589 &  47.278 &  41.400 &                 0.585 &  45.970 &  40.107 &                 0.590 &  47.235 &  43.827 \\
cabinet     &               0.399 &  12.763 &  0.553 &              0.396 &  30.295 &  14.793 &                0.479 &  28.400 &  14.675 &                0.469 &  28.873 &  13.687 &                 0.489 &  32.231 &  18.802 &                 0.486 &  33.080 &  18.931 &                0.504 &  44.310 &  34.230 &                 0.504 &  45.099 &  34.814 &                 0.508 &  42.983 &  33.176 \\
laptop      &               0.514 &   9.666 &  0.319 &              0.512 &  24.325 &  11.004 &                0.576 &  20.907 &   9.476 &                0.557 &  22.173 &   9.603 &                 0.573 &  25.686 &  13.550 &                 0.568 &  27.471 &  15.146 &                0.589 &  38.478 &  28.757 &                 0.585 &  40.640 &  31.472 &                 0.588 &  38.958 &  28.953 \\
bus         &               0.503 &  10.635 &  0.422 &              0.472 &  18.898 &   4.628 &                0.536 &  18.566 &   5.490 &                0.522 &  21.706 &   6.825 &                 0.542 &  29.700 &  15.736 &                 0.534 &  31.953 &  17.941 &                0.568 &  45.085 &  38.868 &                 0.571 &  41.510 &  34.695 &                 0.579 &  39.744 &  33.227 \\
can         &               0.405 &  12.988 &  0.679 &              0.449 &  24.526 &  10.468 &                0.525 &  23.002 &  10.254 &                0.512 &  25.029 &  11.372 &                 0.532 &  28.059 &  14.704 &                 0.532 &  27.866 &  14.448 &                0.547 &  41.839 &  32.118 &                 0.551 &  38.979 &  28.200 &                 0.552 &  39.384 &  30.403 \\
bed         &               0.429 &  13.273 &  0.758 &              0.437 &  21.953 &   6.325 &                0.508 &  20.663 &   7.013 &                0.496 &  21.786 &   7.089 &                 0.514 &  27.184 &  12.194 &                 0.509 &  28.493 &  13.034 &                0.527 &  39.544 &  26.372 &                 0.528 &  40.422 &  27.149 &                 0.530 &  39.752 &  26.920 \\
sofa        &               0.436 &  12.333 &  0.564 &              0.418 &  20.630 &   5.222 &                0.495 &  20.736 &   6.677 &                0.484 &  21.535 &   6.630 &                 0.506 &  29.127 &  14.589 &                 0.503 &  30.679 &  15.634 &                0.532 &  40.797 &  29.990 &                 0.534 &  40.762 &  29.619 &                 0.534 &  40.465 &  30.012 \\
table       &               0.519 &  10.546 &  0.465 &              0.467 &  23.181 &   9.401 &                0.528 &  22.642 &   9.491 &                0.519 &  23.564 &   9.345 &                 0.547 &  28.090 &  13.769 &                 0.544 &  29.031 &  14.291 &                0.580 &  38.306 &  26.010 &                 0.581 &  38.651 &  25.916 &                 0.582 &  37.645 &  25.690 \\
trash       &               0.352 &  14.980 &  0.795 &              0.370 &  24.887 &   8.270 &                0.462 &  23.714 &   8.900 &                0.455 &  25.239 &   9.495 &                 0.474 &  30.569 &  14.939 &                 0.473 &  31.192 &  15.317 &                0.492 &  45.565 &  33.618 &                 0.494 &  43.646 &  31.755 &                 0.496 &  42.358 &  31.069 \\
clock       &               0.444 &  12.433 &  0.620 &              0.425 &  20.866 &   6.133 &                0.515 &  21.335 &   8.267 &                0.508 &  21.661 &   7.726 &                 0.530 &  30.298 &  16.627 &                 0.524 &  31.982 &  17.949 &                0.556 &  49.736 &  44.496 &                 0.559 &  50.434 &  47.352 &                 0.563 &  47.303 &  44.175 \\
skateboard  &               0.653 &   8.237 &  0.279 &              0.617 &  12.328 &   1.778 &                0.642 &  14.552 &   3.505 &                0.624 &  17.254 &   4.499 &                 0.636 &  26.277 &  13.138 &                 0.639 &  25.772 &  12.105 &                0.675 &  35.195 &  27.470 &                 0.688 &  31.216 &  22.573 &                 0.687 &  30.718 &  22.408 \\
mug         &               0.348 &  15.521 &  0.907 &              0.343 &  32.262 &  12.318 &                0.445 &  31.197 &  13.565 &                0.438 &  33.960 &  16.081 &                 0.465 &  36.651 &  20.483 &                 0.463 &  38.786 &  23.104 &                0.485 &  49.002 &  37.643 &                 0.489 &  47.695 &  37.005 &                 0.496 &  45.564 &  36.396 \\
chair       &               0.498 &  11.012 &  0.492 &              0.497 &  17.861 &   4.545 &                0.552 &  18.833 &   6.121 &                0.543 &  19.987 &   6.069 &                 0.559 &  26.972 &  12.162 &                 0.555 &  28.202 &  13.021 &                0.584 &  40.781 &  27.774 &                 0.585 &  40.871 &  27.958 &                 0.590 &  39.552 &  27.345 \\
loudspeaker &               0.400 &  14.026 &  0.780 &              0.405 &  28.105 &  11.770 &                0.492 &  26.560 &  12.239 &                0.483 &  27.262 &  11.825 &                 0.508 &  31.669 &  17.672 &                 0.505 &  32.682 &  18.191 &                0.527 &  45.334 &  35.908 &                 0.529 &  44.613 &  34.268 &                 0.531 &  43.731 &  34.747 \\
camera      &               0.382 &  15.639 &  1.099 &              0.399 &  25.774 &   8.170 &                0.491 &  24.215 &   8.913 &                0.486 &  25.203 &   9.149 &                 0.503 &  29.922 &  14.748 &                 0.504 &  30.999 &  15.706 &                0.520 &  42.891 &  31.324 &                 0.528 &  41.945 &  30.137 &                 0.520 &  42.989 &  33.778 \\
lamp        &               0.639 &   9.868 &  0.641 &              0.613 &  17.295 &   4.709 &                0.663 &  18.762 &   6.118 &                0.654 &  19.730 &   6.496 &                 0.673 &  26.359 &  12.805 &                 0.669 &  27.466 &  13.943 &                0.679 &  42.999 &  36.105 &                 0.686 &  39.772 &  32.010 &                 0.691 &  38.329 &  31.556 \\
airplane    &               0.677 &   7.894 &  0.269 &              0.615 &  15.530 &   3.242 &                0.653 &  19.439 &   6.075 &                0.650 &  21.399 &   7.378 &                 0.674 &  29.746 &  15.845 &                 0.666 &  31.320 &  17.194 &                0.710 &  42.597 &  36.645 &                 0.718 &  39.901 &  33.653 &                 0.719 &  40.058 &  34.923 \\
bag         &               0.467 &  11.503 &  0.528 &              0.440 &  31.729 &  14.865 &                0.515 &  27.381 &  12.217 &                0.510 &  27.431 &  11.845 &                 0.525 &  31.970 &  17.370 &                 0.520 &  32.648 &  17.046 &                0.545 &  47.182 &  38.465 &                 0.554 &  43.010 &  32.777 &                 0.558 &  42.710 &  34.301 \\
car         &               0.383 &  13.588 &  0.636 &              0.386 &  16.711 &   2.038 &                0.466 &  18.057 &   4.978 &                0.457 &  20.808 &   5.734 &                 0.478 &  30.152 &  15.647 &                 0.474 &  32.194 &  17.810 &                0.505 &  44.056 &  36.838 &                 0.507 &  42.851 &  35.437 &                 0.506 &  46.664 &  76.872 \\
bowl        &               0.369 &  14.015 &  0.679 &              0.368 &  16.391 &   2.194 &                0.464 &  19.742 &   5.528 &                0.454 &  21.850 &   6.328 &                 0.492 &  31.341 &  15.914 &                 0.492 &  32.721 &  17.126 &                0.535 &  45.485 &  36.303 &                 0.537 &  42.865 &  32.597 &                 0.539 &  43.340 &  34.686 \\
rocket      &               0.793 &   6.798 &  0.227 &              0.702 &  15.446 &   3.200 &                0.757 &  17.353 &   4.859 &                0.740 &  22.658 &   8.004 &                 0.738 &  32.996 &  19.396 &                 0.714 &  39.521 &  27.271 &                0.727 &  46.225 &  41.530 &                 0.767 &  31.927 &  26.157 &                 0.760 &  34.589 &  29.787 \\
bench       &               0.555 &   9.578 &  0.381 &              0.532 &  14.550 &   3.031 &                0.580 &  16.488 &   4.491 &                0.569 &  17.531 &   4.634 &                 0.593 &  25.561 &  11.605 &                 0.590 &  26.872 &  12.472 &                0.630 &  37.330 &  26.403 &                 0.634 &  36.442 &  24.944 &                 0.630 &  37.055 &  26.275 \\
rifle       &               0.780 &   7.110 &  0.303 &              0.687 &  15.018 &   3.005 &                0.745 &  18.261 &   5.751 &                0.735 &  20.961 &   6.797 &                 0.744 &  29.623 &  16.105 &                 0.729 &  33.845 &  20.096 &                0.748 &  44.706 &  41.341 &                 0.757 &  38.802 &  34.961 &                 0.760 &  37.240 &  33.045 \\
display     &               0.470 &  11.119 &  0.477 &              0.459 &  26.855 &  10.888 &                0.544 &  25.204 &  11.120 &                0.535 &  26.862 &  12.310 &                 0.553 &  30.382 &  16.643 &                 0.547 &  32.515 &  19.081 &                0.573 &  43.438 &  34.554 &                 0.571 &  45.251 &  37.361 &                 0.572 &  44.134 &  36.466 \\
bottle      &               0.549 &   9.733 &  0.370 &              0.543 &  23.363 &   8.833 &                0.580 &  23.325 &   9.651 &                0.575 &  24.030 &   9.645 &                 0.588 &  28.594 &  15.218 &                 0.585 &  29.590 &  16.124 &                0.598 &  49.252 &  45.738 &                 0.609 &  41.510 &  36.607 &                 0.613 &  40.624 &  37.892 \\
mailbox     &               0.635 &   9.133 &  0.388 &              0.640 &  23.528 &  11.404 &                0.688 &  24.145 &  12.649 &                0.679 &  24.823 &  12.807 &                 0.687 &  28.697 &  17.051 &                 0.682 &  29.928 &  17.744 &                0.677 &  43.200 &  35.219 &                 0.682 &  41.354 &  33.328 &                 0.695 &  36.952 &  28.818 \\
motorbike   &               0.422 &  13.439 &  0.751 &              0.435 &  18.641 &   3.065 &                0.503 &  20.897 &   5.364 &                0.499 &  22.325 &   6.106 &                 0.519 &  30.882 &  14.705 &                 0.515 &  33.277 &  16.968 &                0.557 &  45.416 &  36.725 &                 0.561 &  43.878 &  35.158 &                 0.564 &  41.674 &  32.281 \\
faucet      &               0.572 &  10.809 &  0.710 &              0.565 &  18.130 &   4.640 &                0.638 &  20.216 &   6.724 &                0.630 &  21.047 &   6.883 &                 0.657 &  28.851 &  15.064 &                 0.653 &  30.466 &  16.715 &                0.679 &  46.790 &  41.244 &                 0.681 &  44.708 &  39.620 &                 0.694 &  40.844 &  35.357 \\
basket      &               0.382 &  13.828 &  0.726 &              0.372 &  25.477 &   9.355 &                0.474 &  24.792 &  10.701 &                0.465 &  25.840 &  10.762 &                 0.497 &  32.482 &  18.525 &                 0.496 &  32.691 &  18.667 &                0.530 &  43.721 &  34.873 &                 0.534 &  41.407 &  31.708 &                 0.528 &  43.207 &  34.795 \\
file        &               0.395 &  13.222 &  0.629 &              0.394 &  29.136 &  13.066 &                0.473 &  31.093 &  16.589 &                0.465 &  31.363 &  15.231 &                 0.487 &  35.883 &  22.353 &                 0.484 &  36.623 &  21.885 &                0.503 &  47.757 &  37.984 &                 0.501 &  50.006 &  40.969 &                 0.508 &  46.453 &  37.485 \\
birdhouse   &               0.379 &  15.464 &  0.976 &              0.388 &  30.077 &  11.390 &                0.478 &  31.029 &  14.332 &                0.472 &  32.213 &  14.811 &                 0.493 &  36.573 &  21.478 &                 0.492 &  38.760 &  23.960 &                0.513 &  51.745 &  44.294 &                 0.515 &  50.632 &  42.667 &                 0.516 &  48.789 &  41.969 \\
knife       &               0.851 &   6.013 &  0.196 &              0.819 &  13.634 &   4.026 &                0.805 &  16.790 &   5.387 &                0.798 &  16.917 &   5.025 &                 0.796 &  23.943 &  11.163 &                 0.790 &  24.760 &  12.290 &                0.771 &  43.403 &  41.529 &                 0.777 &  37.949 &  33.881 &                 0.795 &  33.139 &  29.773 \\
flowerpot   &               0.394 &  15.280 &  1.014 &              0.395 &  23.128 &   6.366 &                0.490 &  23.584 &   8.337 &                0.483 &  24.486 &   8.654 &                 0.509 &  31.493 &  15.703 &                 0.506 &  33.069 &  16.914 &                0.535 &  47.611 &  37.441 &                 0.538 &  45.750 &  35.489 &                 0.541 &  44.383 &  35.139 \\
pistol      &               0.590 &   9.613 &  0.431 &              0.560 &  16.331 &   3.434 &                0.622 &  19.507 &   6.373 &                0.613 &  21.672 &   7.002 &                 0.624 &  32.368 &  18.467 &                 0.611 &  36.355 &  23.262 &                0.638 &  56.032 &  60.739 &                 0.647 &  47.114 &  44.447 &                 0.654 &  44.805 &  41.385 \\
piano       &               0.423 &  13.205 &  0.765 &              0.441 &  27.252 &  10.404 &                0.511 &  26.458 &  11.034 &                0.501 &  26.845 &  10.711 &                 0.523 &  29.922 &  15.477 &                 0.519 &  31.362 &  16.052 &                0.547 &  42.677 &  31.710 &                 0.546 &  43.403 &  33.516 &                 0.540 &  44.174 &  35.012 \\
dishwasher  &               0.390 &  12.902 &  0.553 &              0.447 &  38.225 &  26.598 &                0.515 &  39.390 &  27.329 &                0.501 &  36.872 &  22.944 &                 0.524 &  41.641 &  30.542 &                 0.519 &  42.344 &  29.520 &                0.527 &  51.921 &  45.119 &                 0.527 &  50.051 &  42.309 &                 0.531 &  48.802 &  42.539 \\
remote      &               0.565 &   9.499 &  0.357 &              0.540 &  18.916 &   6.342 &                0.614 &  17.593 &   6.190 &                0.605 &  18.057 &   5.786 &                 0.601 &  25.195 &  11.715 &                 0.591 &  25.558 &  11.469 &                0.612 &  38.923 &  27.942 &                 0.618 &  39.983 &  32.706 &                 0.623 &  37.443 &  30.462 \\
keyboard    &               0.576 &   8.743 &  0.296 &              0.551 &  10.459 &   0.711 &                0.583 &  16.492 &   4.797 &                0.573 &  17.389 &   5.070 &                 0.596 &  26.925 &  14.705 &                 0.610 &  25.163 &  13.432 &                0.651 &  38.141 &  31.050 &                 0.658 &  34.705 &  26.464 &                 0.616 &  42.261 &  36.788 \\
\midrule
mean        &               0.497 &  11.622 &  0.577 &              0.485 &  22.296 &   7.880 &                0.555 &  22.846 &   9.260 &                0.546 &  23.988 &   9.444 &                 0.565 &  30.420 &  16.503 &                 0.561 &  31.866 &  17.746 &                0.585 &  44.629 &  36.697 &                 0.589 &  42.531 &  34.114 &                 0.592 &  41.683 &  34.890 \\
\bottomrule
\end{tabular}

==> tables/baseline_all_augmented_data_cdl1.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
\multirow{2}[3]{*}{Object} & \multicolumn{2}{c}{R: $25^\circ$, T: 0} &  \multicolumn{2}{c}{R: $25^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $180^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.5}\\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} 
{} & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr  & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours \\
\midrule
airplane    &                 20.799 &             15.530 &                   24.766 &               19.439 &                   27.298 &               21.399 &                    35.288 &                29.746 &                    35.542 &                31.320 &                   48.002 &               42.597 &                    47.655 &                39.901 &                    47.216 &                40.058 \\
bag         &                 28.086 &             31.729 &                   30.164 &               27.381 &                   29.927 &               27.431 &                    38.678 &                31.970 &                    38.250 &                32.648 &                   55.111 &               47.182 &                    56.556 &                43.010 &                    56.962 &                42.710 \\
basket      &                 26.186 &             25.477 &                   28.179 &               24.792 &                   28.227 &               25.840 &                    37.330 &                32.482 &                    37.339 &                32.691 &                   51.428 &               43.721 &                    51.198 &                41.407 &                    52.894 &                43.207 \\
bathtub     &                 22.955 &             21.281 &                   25.353 &               22.000 &                   26.157 &               22.110 &                    33.855 &                28.839 &                    34.791 &                30.468 &                   46.787 &               40.885 &                    46.189 &                39.767 &                    46.012 &                39.785 \\
bed         &                 23.458 &             21.953 &                   24.096 &               20.663 &                   24.962 &               21.786 &                    31.255 &                27.184 &                    32.361 &                28.493 &                   44.216 &               39.544 &                    43.284 &                40.422 &                    43.679 &                39.752 \\
bench       &                 17.583 &             14.550 &                   21.413 &               16.488 &                   21.902 &               17.531 &                    31.925 &                25.561 &                    32.373 &                26.872 &                   46.099 &               37.330 &                    47.172 &                36.442 &                    44.633 &                37.055 \\
birdhouse   &                 31.957 &             30.077 &                   32.975 &               31.029 &                   32.700 &               32.213 &                    37.369 &                36.573 &                    37.673 &                38.760 &                   47.231 &               51.745 &                    48.902 &                50.632 &                    47.654 &                48.789 \\
bookshelf   &                 22.588 &             21.933 &                   25.536 &               21.255 &                   25.815 &               22.561 &                    36.407 &                31.215 &                    35.995 &                32.256 &                   51.990 &               46.621 &                    48.066 &                45.490 &                    50.803 &                45.120 \\
bottle      &                 20.826 &             23.363 &                   23.460 &               23.325 &                   23.460 &               24.030 &                    32.090 &                28.594 &                    32.204 &                29.590 &                   48.711 &               49.252 &                    48.335 &                41.510 &                    48.473 &                40.624 \\
bowl        &                 16.810 &             16.391 &                   24.027 &               19.742 &                   24.080 &               21.850 &                    38.692 &                31.341 &                    38.565 &                32.721 &                   54.995 &               45.485 &                    55.099 &                42.865 &                    54.822 &                43.340 \\
bus         &                 19.819 &             18.898 &                   23.900 &               18.566 &                   25.420 &               21.706 &                    34.753 &                29.700 &                    36.576 &                31.953 &                   50.625 &               45.085 &                    49.179 &                41.510 &                    49.377 &                39.744 \\
cabinet     &                 32.240 &             30.295 &                   33.780 &               28.400 &                   34.025 &               28.873 &                    39.668 &                32.231 &                    39.485 &                33.080 &                   51.768 &               44.310 &                    51.573 &                45.099 &                    50.882 &                42.983 \\
camera      &                 28.292 &             25.774 &                   32.992 &               24.215 &                   34.095 &               25.203 &                    43.744 &                29.922 &                    43.695 &                30.999 &                   59.438 &               42.891 &                    58.758 &                41.945 &                    59.947 &                42.989 \\
can         &                 22.013 &             24.526 &                   23.488 &               23.002 &                   23.437 &               25.029 &                    30.281 &                28.059 &                    30.154 &                27.866 &                   46.481 &               41.839 &                    46.623 &                38.979 &                    46.628 &                39.384 \\
cap         &                 20.701 &             17.737 &                   24.447 &               20.816 &                   25.339 &               23.424 &                    32.291 &                33.220 &                    34.176 &                33.683 &                   46.590 &               47.278 &                    48.523 &                45.970 &                    45.689 &                47.235 \\
car         &                 18.764 &             16.711 &                   23.920 &               18.057 &                   25.166 &               20.808 &                    36.887 &                30.152 &                    37.359 &                32.194 &                   52.451 &               44.056 &                    51.048 &                42.851 &                    51.427 &                46.664 \\
cellphone   &                 20.553 &             20.226 &                   25.244 &               20.980 &                   25.942 &               21.179 &                    36.031 &                28.946 &                    36.800 &                29.751 &                   53.874 &               45.535 &                    51.355 &                47.679 &                    55.647 &                43.722 \\
chair       &                 20.618 &             17.861 &                   23.204 &               18.833 &                   24.504 &               19.987 &                    32.613 &                26.972 &                    33.192 &                28.202 &                   46.026 &               40.781 &                    46.424 &                40.871 &                    46.583 &                39.552 \\
clock       &                 22.903 &             20.866 &                   27.920 &               21.335 &                   28.573 &               21.661 &                    39.362 &                30.298 &                    40.984 &                31.982 &                   58.713 &               49.736 &                    57.499 &                50.434 &                    59.874 &                47.303 \\
dishwasher  &                 38.851 &             38.225 &                   40.459 &               39.390 &                   40.107 &               36.872 &                    43.130 &                41.641 &                    42.843 &                42.344 &                   49.208 &               51.921 &                    49.399 &                50.051 &                    49.513 &                48.802 \\
display     &                 28.698 &             26.855 &                   31.285 &               25.204 &                   32.157 &               26.862 &                    40.230 &                30.382 &                    42.074 &                32.515 &                   57.058 &               43.438 &                    53.920 &                45.251 &                    53.920 &                44.134 \\
earphone    &                 20.002 &             17.639 &                   25.072 &               19.435 &                   26.125 &               21.576 &                    35.779 &                28.667 &                    34.298 &                29.995 &                   45.332 &               44.597 &                    50.272 &                42.063 &                    48.314 &                39.620 \\
faucet      &                 19.901 &             18.130 &                   23.760 &               20.216 &                   25.399 &               21.047 &                    34.760 &                28.851 &                    36.060 &                30.466 &                   48.872 &               46.790 &                    48.970 &                44.708 &                    45.329 &                40.844 \\
file        &                 31.172 &             29.136 &                   32.783 &               31.093 &                   33.005 &               31.363 &                    39.809 &                35.883 &                    40.075 &                36.623 &                   52.652 &               47.757 &                    49.632 &                50.006 &                    53.266 &                46.453 \\
flowerpot   &                 24.210 &             23.128 &                   26.937 &               23.584 &                   27.173 &               24.486 &                    36.594 &                31.493 &                    36.433 &                33.069 &                   53.507 &               47.611 &                    52.546 &                45.750 &                    52.303 &                44.383 \\
guitar      &                 14.724 &             15.582 &                   20.592 &               20.082 &                   20.598 &               18.538 &                    30.649 &                27.481 &                    31.318 &                27.529 &                   49.012 &               45.950 &                    47.942 &                39.648 &                    48.927 &                37.818 \\
helmet      &                 23.659 &             23.051 &                   28.153 &               24.310 &                   29.078 &               26.828 &                    40.104 &                35.526 &                    41.105 &                36.940 &                   57.753 &               51.349 &                    56.712 &                49.150 &                    56.767 &                48.334 \\
jar         &                 20.562 &             20.701 &                   24.981 &               20.755 &                   25.022 &               21.915 &                    35.680 &                28.488 &                    35.694 &                29.609 &                   53.251 &               47.355 &                    53.533 &                43.768 &                    53.399 &                42.144 \\
keyboard    &                 11.502 &             10.459 &                   17.487 &               16.492 &                   17.916 &               17.389 &                    28.383 &                26.925 &                    29.684 &                25.163 &                   42.436 &               38.141 &                    41.689 &                34.705 &                    45.218 &                42.261 \\
knife       &                 13.404 &             13.634 &                   16.559 &               16.790 &                   16.770 &               16.917 &                    24.068 &                23.943 &                    24.010 &                24.760 &                   38.505 &               43.403 &                    37.067 &                37.949 &                    38.449 &                33.139 \\
lamp        &                 17.379 &             17.295 &                   21.169 &               18.762 &                   21.564 &               19.730 &                    30.582 &                26.359 &                    31.112 &                27.466 &                   46.214 &               42.999 &                    46.368 &                39.772 &                    46.511 &                38.329 \\
laptop      &                 23.755 &             24.325 &                   25.061 &               20.907 &                   25.557 &               22.173 &                    32.562 &                25.686 &                    33.745 &                27.471 &                   49.101 &               38.478 &                    49.667 &                40.640 &                    46.924 &                38.958 \\
loudspeaker &                 29.544 &             28.105 &                   31.092 &               26.560 &                   31.211 &               27.262 &                    37.735 &                31.669 &                    37.960 &                32.682 &                   51.196 &               45.334 &                    51.627 &                44.613 &                    51.891 &                43.731 \\
mailbox     &                 23.032 &             23.528 &                   23.196 &               24.145 &                   23.143 &               24.823 &                    26.917 &                28.697 &                    26.667 &                29.928 &                   37.997 &               43.200 &                    38.208 &                41.354 &                    39.097 &                36.952 \\
microphone  &                 19.403 &             19.876 &                   23.093 &               20.077 &                   24.031 &               20.928 &                    34.140 &                24.763 &                    35.507 &                28.295 &                   54.367 &               37.941 &                    54.199 &                34.210 &                    53.123 &                34.434 \\
microwaves  &                 43.955 &             44.618 &                   43.753 &               41.156 &                   44.239 &               40.319 &                    45.676 &                41.447 &                    45.186 &                42.166 &                   49.152 &               46.961 &                    47.830 &                46.193 &                    46.464 &                46.741 \\
motorbike   &                 20.391 &             18.641 &                   25.736 &               20.897 &                   26.891 &               22.325 &                    38.518 &                30.882 &                    40.309 &                33.277 &                   56.563 &               45.416 &                    52.141 &                43.878 &                    48.685 &                41.674 \\
mug         &                 31.494 &             32.262 &                   34.490 &               31.197 &                   36.622 &               33.960 &                    44.299 &                36.651 &                    44.851 &                38.786 &                   59.581 &               49.002 &                    58.508 &                47.695 &                    59.635 &                45.564 \\
piano       &                 29.632 &             27.252 &                   32.755 &               26.458 &                   33.911 &               26.845 &                    40.862 &                29.922 &                    41.922 &                31.362 &                   53.421 &               42.677 &                    52.878 &                43.403 &                    48.535 &                44.174 \\
pillow      &                 16.006 &             13.710 &                   19.679 &               16.000 &                   20.055 &               17.371 &                    31.062 &                27.507 &                    30.944 &                28.532 &                   45.539 &               40.643 &                    45.386 &                40.373 &                    46.354 &                39.725 \\
pistol      &                 17.872 &             16.331 &                   23.967 &               19.507 &                   25.460 &               21.672 &                    35.656 &                32.368 &                    37.386 &                36.355 &                   51.641 &               56.032 &                    49.420 &                47.114 &                    55.810 &                44.805 \\
printer     &                 30.877 &             30.601 &                   31.076 &               27.563 &                   31.801 &               27.793 &                    37.578 &                30.729 &                    37.149 &                32.724 &                   47.604 &               43.124 &                    46.687 &                43.954 &                    48.345 &                42.179 \\
remote      &                 20.743 &             18.916 &                   22.540 &               17.593 &                   23.036 &               18.057 &                    30.893 &                25.195 &                    30.933 &                25.558 &                   47.288 &               38.923 &                    48.908 &                39.983 &                    51.606 &                37.443 \\
rifle       &                 15.380 &             15.018 &                   21.375 &               18.261 &                   23.435 &               20.961 &                    33.520 &                29.623 &                    35.245 &                33.845 &                   49.443 &               44.706 &                    47.069 &                38.802 &                    46.274 &                37.240 \\
rocket      &                 16.237 &             15.446 &                   20.474 &               17.353 &                   25.746 &               22.658 &                    31.895 &                32.996 &                    36.251 &                39.521 &                   44.888 &               46.225 &                    51.728 &                31.927 &                    46.071 &                34.589 \\
skateboard  &                 15.121 &             12.328 &                   18.941 &               14.552 &                   19.141 &               17.254 &                    29.690 &                26.277 &                    30.042 &                25.772 &                   48.058 &               35.195 &                    45.425 &                31.216 &                    46.527 &                30.718 \\
sofa        &                 22.789 &             20.630 &                   25.665 &               20.736 &                   26.267 &               21.535 &                    34.804 &                29.127 &                    35.229 &                30.679 &                   47.488 &               40.797 &                    47.583 &                40.762 &                    47.738 &                40.465 \\
stove       &                 31.083 &             31.492 &                   32.292 &               30.239 &                   32.277 &               29.905 &                    37.076 &                32.611 &                    37.392 &                34.107 &                   47.998 &               45.759 &                    47.593 &                43.722 &                    47.827 &                43.602 \\
table       &                 24.619 &             23.181 &                   25.633 &               22.642 &                   26.270 &               23.564 &                    32.851 &                28.090 &                    32.881 &                29.031 &                   44.154 &               38.306 &                    44.490 &                38.651 &                    44.398 &                37.645 \\
telephone   &                 19.905 &             19.543 &                   25.080 &               21.485 &                   25.888 &               21.374 &                    36.732 &                29.911 &                    38.047 &                31.115 &                   56.734 &               47.336 &                    56.665 &                47.090 &                    54.820 &                45.154 \\
tower       &                 20.365 &             22.278 &                   22.988 &               22.677 &                   23.319 &               23.229 &                    31.359 &                29.829 &                    31.485 &                31.612 &                   50.122 &               46.606 &                    50.136 &                41.206 &                    46.853 &                41.147 \\
train       &                 19.035 &             18.138 &                   22.941 &               19.800 &                   24.427 &               22.396 &                    34.463 &                31.132 &                    35.758 &                33.632 &                   53.302 &               45.224 &                    50.006 &                43.613 &                    49.148 &                42.028 \\
trash       &                 25.162 &             24.887 &                   27.930 &               23.714 &                   28.071 &               25.239 &                    35.697 &                30.569 &                    35.693 &                31.192 &                   50.538 &               45.565 &                    50.596 &                43.646 &                    50.861 &                42.358 \\
washer      &                 37.960 &             37.926 &                   39.529 &               36.989 &                   39.715 &               37.528 &                    44.605 &                39.109 &                    43.430 &                38.926 &                   54.986 &               46.540 &                    56.116 &                45.058 &                    55.478 &                45.971 \\
watercraft  &                 19.564 &             18.230 &                   22.921 &               19.610 &                   24.492 &               22.021 &                    33.044 &                29.666 &                    34.466 &                34.034 &                   48.829 &               47.429 &                    50.306 &                40.480 &                    50.110 &                38.979 \\
\midrule
mean        &                 23.184 &             22.296 &                   26.369 &               22.846 &                   27.108 &               23.988 &                    35.453 &                30.420 &                    36.013 &                31.866 &                   50.079 &               44.629 &                    49.721 &                42.531 &                    49.703 &                41.683 \\
\bottomrule
\end{tabular}

==> tables/baseline_all_augmented_data_cdl2.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
\multirow{2}[3]{*}{Object} & \multicolumn{2}{c}{R: $25^\circ$, T: 0} &  \multicolumn{2}{c}{R: $25^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $180^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.5}\\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} 
{} & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr  & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours \\
\midrule
airplane    &                  5.641 &              3.242 &                    8.072 &                6.075 &                   10.282 &                7.378 &                    18.841 &                15.845 &                    19.463 &                17.194 &                   40.535 &               36.645 &                    39.816 &                33.653 &                    39.407 &                34.923 \\
bag         &                  9.643 &             14.865 &                   11.422 &               12.217 &                   11.146 &               11.845 &                    19.357 &                17.370 &                    18.814 &                17.046 &                   41.992 &               38.465 &                    45.845 &                32.777 &                    48.244 &                34.301 \\
basket      &                  9.089 &              9.355 &                    9.533 &               10.701 &                    9.324 &               10.762 &                    16.341 &                18.525 &                    16.345 &                18.667 &                   34.912 &               34.873 &                    34.284 &                31.708 &                    36.350 &                34.795 \\
bathtub     &                  5.928 &              5.970 &                    7.611 &                7.708 &                    8.008 &                7.342 &                    15.011 &                14.432 &                    16.191 &                15.751 &                   32.497 &               30.172 &                    31.915 &                28.461 &                    31.683 &                30.022 \\
bed         &                  6.227 &              6.325 &                    6.550 &                7.013 &                    6.898 &                7.089 &                    12.004 &                12.194 &                    12.905 &                13.034 &                   26.792 &               26.372 &                    25.829 &                27.149 &                    26.006 &                26.920 \\
bench       &                  3.619 &              3.031 &                    5.483 &                4.491 &                    5.668 &                4.634 &                    13.103 &                11.605 &                    13.391 &                12.472 &                   30.702 &               26.403 &                    32.324 &                24.944 &                    29.465 &                26.275 \\
birdhouse   &                 11.926 &             11.390 &                   12.651 &               14.332 &                   12.314 &               14.811 &                    16.681 &                21.478 &                    17.005 &                23.960 &                   28.555 &               44.294 &                    30.625 &                42.667 &                    29.855 &                41.969 \\
bookshelf   &                  6.373 &              7.296 &                    7.905 &                7.769 &                    7.659 &                7.811 &                    16.104 &                16.663 &                    15.432 &                16.992 &                   35.566 &               36.757 &                    30.929 &                34.487 &                    34.106 &                36.040 \\
bottle      &                  6.159 &              8.833 &                    7.384 &                9.651 &                    7.395 &                9.645 &                    14.845 &                15.218 &                    15.021 &                16.124 &                   37.412 &               45.738 &                    36.955 &                36.607 &                    37.135 &                37.892 \\
bowl        &                  2.083 &              2.194 &                    5.670 &                5.528 &                    5.733 &                6.328 &                    18.724 &                15.914 &                    18.523 &                17.126 &                   43.120 &               36.303 &                    43.091 &                32.597 &                    42.785 &                34.686 \\
bus         &                  4.217 &              4.628 &                    6.848 &                5.490 &                    7.615 &                6.825 &                    16.451 &                15.736 &                    18.708 &                17.941 &                   40.055 &               38.868 &                    38.484 &                34.695 &                    39.324 &                33.227 \\
cabinet     &                 13.784 &             14.793 &                   15.375 &               14.675 &                   14.784 &               13.687 &                    20.901 &                18.802 &                    20.527 &                18.931 &                   37.685 &               34.230 &                    37.183 &                34.814 &                    36.458 &                33.176 \\
camera      &                  8.671 &              8.170 &                   12.933 &                8.913 &                   13.717 &                9.149 &                    24.424 &                14.748 &                    23.972 &                15.706 &                   49.689 &               31.324 &                    48.229 &                30.137 &                    50.670 &                33.778 \\
can         &                  7.458 &             10.468 &                    8.049 &               10.254 &                    7.983 &               11.372 &                    12.315 &                14.704 &                    12.274 &                14.448 &                   29.987 &               32.118 &                    30.145 &                28.200 &                    30.142 &                30.403 \\
cap         &                  4.491 &              3.610 &                    7.478 &                7.230 &                    7.932 &                8.361 &                    15.278 &                18.782 &                    16.563 &                19.614 &                   34.153 &               41.400 &                    37.039 &                40.107 &                    35.001 &                43.827 \\
car         &                  2.456 &              2.038 &                    6.000 &                4.978 &                    6.677 &                5.734 &                    17.614 &                15.647 &                    18.374 &                17.810 &                   41.340 &               36.838 &                    39.831 &                35.437 &                    40.402 &                76.872 \\
cellphone   &                  4.934 &              6.360 &                    7.107 &                7.910 &                    7.134 &                7.206 &                    16.111 &                15.216 &                    16.949 &                15.821 &                   42.547 &               38.399 &                    38.862 &                42.926 &                    45.366 &                38.341 \\
chair       &                  5.140 &              4.545 &                    6.640 &                6.121 &                    7.345 &                6.069 &                    13.398 &                12.162 &                    13.891 &                13.021 &                   28.852 &               27.774 &                    29.671 &                27.958 &                    29.754 &                27.345 \\
clock       &                  5.888 &              6.133 &                    8.700 &                8.267 &                    8.963 &                7.726 &                    19.577 &                16.627 &                    21.616 &                17.949 &                   48.808 &               44.496 &                    46.267 &                47.352 &                    52.733 &                44.175 \\
dishwasher  &                 23.804 &             26.598 &                   26.189 &               27.329 &                   25.186 &               22.944 &                    29.978 &                30.542 &                    28.885 &                29.520 &                   39.590 &               45.119 &                    39.454 &                42.309 &                    39.170 &                42.539 \\
display     &                 10.939 &             10.888 &                   12.555 &               11.120 &                   13.026 &               12.310 &                    20.915 &                16.643 &                    23.885 &                19.081 &                   46.820 &               34.554 &                    41.680 &                37.361 &                    41.124 &                36.466 \\
earphone    &                  4.032 &              3.283 &                    6.959 &                5.350 &                    7.591 &                6.282 &                    15.781 &                13.019 &                    14.575 &                14.313 &                   31.581 &               37.056 &                    37.219 &                31.383 &                    32.219 &                28.464 \\
faucet      &                  5.044 &              4.640 &                    7.247 &                6.724 &                    8.542 &                6.883 &                    17.066 &                15.064 &                    18.798 &                16.715 &                   37.415 &               41.244 &                    38.045 &                39.620 &                    33.620 &                35.357 \\
file        &                 12.687 &             13.066 &                   14.298 &               16.589 &                   13.958 &               15.231 &                    20.664 &                22.353 &                    21.111 &                21.885 &                   39.141 &               37.984 &                    35.298 &                40.969 &                    40.218 &                37.485 \\
flowerpot   &                  6.218 &              6.366 &                    7.680 &                8.337 &                    7.768 &                8.654 &                    15.333 &                15.703 &                    15.200 &                16.914 &                   37.411 &               37.441 &                    35.830 &                35.489 &                    35.611 &                35.139 \\
guitar      &                  3.031 &              3.826 &                    5.660 &                6.516 &                    5.600 &                5.857 &                    14.332 &                14.194 &                    14.487 &                13.989 &                   39.831 &               41.859 &                    38.201 &                34.128 &                    39.889 &                34.205 \\
helmet      &                  4.848 &              5.350 &                    7.611 &                7.949 &                    8.102 &                9.754 &                    18.500 &                19.604 &                    19.524 &                20.848 &                   43.436 &               41.359 &                    42.801 &                38.449 &                    42.516 &                39.469 \\
jar         &                  4.571 &              5.225 &                    6.585 &                6.242 &                    6.606 &                6.632 &                    14.991 &                13.090 &                    15.006 &                13.964 &                   38.566 &               38.203 &                    38.876 &                33.467 &                    38.753 &                33.042 \\
keyboard    &                  0.886 &              0.711 &                    5.211 &                4.797 &                    5.223 &                5.070 &                    15.983 &                14.705 &                    16.609 &                13.432 &                   34.377 &               31.050 &                    32.580 &                26.464 &                    36.546 &                36.788 \\
knife       &                  4.077 &              4.026 &                    4.420 &                5.387 &                    4.573 &                5.025 &                     9.703 &                11.163 &                     9.875 &                12.290 &                   28.280 &               41.529 &                    26.806 &                33.881 &                    28.218 &                29.773 \\
lamp        &                  4.271 &              4.709 &                    5.838 &                6.118 &                    6.053 &                6.496 &                    13.173 &                12.805 &                    13.904 &                13.943 &                   34.449 &               36.105 &                    34.784 &                32.010 &                    35.091 &                31.556 \\
laptop      &                  9.375 &             11.004 &                   10.507 &                9.476 &                   10.359 &                9.603 &                    16.991 &                13.550 &                    17.716 &                15.146 &                   38.080 &               28.757 &                    38.244 &                31.472 &                    35.250 &                28.953 \\
loudspeaker &                 10.976 &             11.770 &                   12.370 &               12.239 &                   11.942 &               11.825 &                    18.505 &                17.672 &                    18.455 &                18.191 &                   36.733 &               35.908 &                    37.385 &                34.268 &                    37.140 &                34.747 \\
mailbox     &                 10.035 &             11.404 &                    9.909 &               12.649 &                    9.627 &               12.807 &                    12.638 &                17.051 &                    12.263 &                17.744 &                   24.600 &               35.219 &                    25.071 &                33.328 &                    25.503 &                28.818 \\
microphone  &                  5.572 &              6.732 &                    7.423 &                7.271 &                    8.307 &                7.854 &                    17.593 &                11.391 &                    20.404 &                14.333 &                   46.579 &               28.814 &                    48.349 &                26.889 &                    45.186 &                29.081 \\
microwaves  &                 25.961 &             28.869 &                   26.507 &               27.348 &                   25.817 &               26.065 &                    28.594 &                29.498 &                    27.741 &                30.388 &                   35.612 &               38.837 &                    32.951 &                36.262 &                    31.624 &                39.347 \\
motorbike   &                  3.636 &              3.065 &                    6.398 &                5.364 &                    7.278 &                6.106 &                    17.224 &                14.705 &                    20.217 &                16.968 &                   46.168 &               36.725 &                    38.948 &                35.158 &                    33.905 &                32.281 \\
mug         &                 10.976 &             12.318 &                   13.290 &               13.565 &                   15.782 &               16.081 &                    22.912 &                20.483 &                    24.729 &                23.104 &                   44.687 &               37.643 &                    44.368 &                37.005 &                    45.539 &                36.396 \\
piano       &                 10.417 &             10.404 &                   13.227 &               11.034 &                   13.612 &               10.711 &                    21.350 &                15.477 &                    21.997 &                16.052 &                   39.084 &               31.710 &                    39.750 &                33.516 &                    33.316 &                35.012 \\
pillow      &                  1.647 &              1.208 &                    3.431 &                3.389 &                    3.611 &                3.971 &                    14.042 &                14.936 &                    13.931 &                15.588 &                   35.608 &               34.230 &                    35.761 &                32.655 &                    35.340 &                33.412 \\
pistol      &                  3.644 &              3.434 &                    6.802 &                6.373 &                    7.687 &                7.002 &                    17.103 &                18.467 &                    20.337 &                23.262 &                   43.044 &               60.739 &                    41.690 &                44.447 &                    50.084 &                41.385 \\
printer     &                 11.911 &             12.730 &                   12.377 &               12.394 &                   12.514 &               11.866 &                    18.219 &                17.032 &                    17.576 &                18.598 &                   31.527 &               33.371 &                    30.359 &                33.826 &                    32.827 &                31.680 \\
remote      &                  5.997 &              6.342 &                    7.511 &                6.190 &                    7.422 &                5.786 &                    14.756 &                11.715 &                    14.045 &                11.469 &                   36.547 &               27.942 &                    40.202 &                32.706 &                    44.594 &                30.462 \\
rifle       &                  3.187 &              3.005 &                    6.080 &                5.751 &                    7.423 &                6.797 &                    16.627 &                16.105 &                    19.875 &                20.096 &                   42.923 &               41.341 &                    39.953 &                34.961 &                    39.210 &                33.045 \\
rocket      &                  3.390 &              3.200 &                    5.076 &                4.859 &                    8.102 &                8.004 &                    13.555 &                19.396 &                    20.783 &                27.271 &                   36.405 &               41.530 &                    43.797 &                26.157 &                    38.928 &                29.787 \\
skateboard  &                  2.522 &              1.778 &                    5.061 &                3.505 &                    5.245 &                4.499 &                    14.784 &                13.138 &                    14.810 &                12.105 &                   39.777 &               27.470 &                    38.744 &                22.573 &                    39.053 &                22.408 \\
sofa        &                  5.447 &              5.222 &                    7.545 &                6.677 &                    7.756 &                6.630 &                    15.467 &                14.589 &                    15.809 &                15.634 &                   32.724 &               29.990 &                    32.394 &                29.619 &                    32.870 &                30.012 \\
stove       &                 14.735 &             15.931 &                   15.829 &               17.307 &                   15.557 &               15.831 &                    20.387 &                20.117 &                    20.405 &                21.168 &                   35.308 &               37.122 &                    34.678 &                34.472 &                    35.418 &                36.000 \\
table       &                  8.864 &              9.401 &                    9.348 &                9.491 &                    9.597 &                9.345 &                    14.851 &                13.769 &                    14.899 &                14.291 &                   28.407 &               26.010 &                    28.701 &                25.916 &                    28.687 &                25.690 \\
telephone   &                  4.639 &              5.969 &                    6.887 &                8.302 &                    7.067 &                7.469 &                    16.380 &                16.347 &                    17.926 &                17.578 &                   46.076 &               41.487 &                    45.835 &                41.580 &                    42.231 &                41.228 \\
tower       &                  5.718 &              7.744 &                    7.061 &                9.195 &                    7.276 &                9.350 &                    13.837 &                16.582 &                    14.287 &                18.772 &                   39.689 &               41.516 &                    41.123 &                34.379 &                    35.401 &                37.263 \\
train       &                  3.885 &              4.232 &                    5.901 &                6.010 &                    6.624 &                6.981 &                    15.991 &                16.889 &                    17.766 &                19.024 &                   44.892 &               40.279 &                    39.980 &                39.422 &                    39.514 &                38.957 \\
trash       &                  7.584 &              8.270 &                    9.184 &                8.900 &                    9.170 &                9.495 &                    15.105 &                14.939 &                    15.205 &                15.317 &                   33.872 &               33.618 &                    34.195 &                31.755 &                    34.519 &                31.069 \\
washer      &                 20.274 &             22.758 &                   21.961 &               23.603 &                   21.452 &               22.842 &                    27.421 &                27.096 &                    25.900 &                26.231 &                   41.826 &               37.752 &                    43.399 &                35.580 &                    43.017 &                38.084 \\
watercraft  &                  4.861 &              4.669 &                    6.980 &                6.649 &                    8.050 &                7.574 &                    16.117 &                16.174 &                    18.217 &                21.190 &                   40.511 &               45.334 &                    42.835 &                36.094 &                    43.117 &                34.600 \\
\midrule
mean        &                  7.334 &              7.880 &                    9.242 &                9.260 &                    9.565 &                9.444 &                    17.163 &                16.503 &                    17.875 &                17.746 &                   37.760 &               36.697 &                    37.411 &                34.114 &                    37.457 &                34.890 \\
\bottomrule
\end{tabular}

==> tables/baseline_all_augmented_data_fscore.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
\multirow{2}[3]{*}{Object} & \multicolumn{2}{c}{R: $25^\circ$, T: 0} &  \multicolumn{2}{c}{R: $25^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.1} & \multicolumn{2}{c}{R: $45^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.25} & \multicolumn{2}{c}{R: $90^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $180^\circ$, T: 0.5} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.5}\\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} 
{} & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr  & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours & PoinTr & Ours \\
\midrule
airplane    &                  0.578 &              0.615 &                    0.567 &                0.653 &                    0.560 &                0.650 &                     0.575 &                 0.674 &                     0.575 &                 0.666 &                    0.603 &                0.710 &                     0.604 &                 0.718 &                     0.605 &                 0.719 \\
bag         &                  0.412 &              0.440 &                    0.408 &                0.515 &                    0.410 &                0.510 &                     0.413 &                 0.525 &                     0.410 &                 0.520 &                    0.429 &                0.545 &                     0.433 &                 0.554 &                     0.431 &                 0.558 \\
basket      &                  0.370 &              0.372 &                    0.367 &                0.474 &                    0.365 &                0.465 &                     0.374 &                 0.497 &                     0.372 &                 0.496 &                    0.397 &                0.530 &                     0.401 &                 0.534 &                     0.401 &                 0.528 \\
bathtub     &                  0.401 &              0.429 &                    0.404 &                0.501 &                    0.401 &                0.492 &                     0.410 &                 0.518 &                     0.409 &                 0.515 &                    0.429 &                0.547 &                     0.430 &                 0.551 &                     0.429 &                 0.552 \\
bed         &                  0.416 &              0.437 &                    0.421 &                0.508 &                    0.418 &                0.496 &                     0.423 &                 0.514 &                     0.419 &                 0.509 &                    0.427 &                0.527 &                     0.425 &                 0.528 &                     0.424 &                 0.530 \\
bench       &                  0.492 &              0.532 &                    0.490 &                0.580 &                    0.484 &                0.569 &                     0.490 &                 0.593 &                     0.488 &                 0.590 &                    0.512 &                0.630 &                     0.511 &                 0.634 &                     0.518 &                 0.630 \\
birdhouse   &                  0.371 &              0.388 &                    0.369 &                0.478 &                    0.368 &                0.472 &                     0.374 &                 0.493 &                     0.376 &                 0.492 &                    0.391 &                0.513 &                     0.388 &                 0.515 &                     0.396 &                 0.516 \\
bookshelf   &                  0.384 &              0.400 &                    0.385 &                0.486 &                    0.381 &                0.477 &                     0.387 &                 0.496 &                     0.386 &                 0.494 &                    0.407 &                0.519 &                     0.414 &                 0.523 &                     0.411 &                 0.524 \\
bottle      &                  0.519 &              0.543 &                    0.485 &                0.580 &                    0.485 &                0.575 &                     0.470 &                 0.588 &                     0.470 &                 0.585 &                    0.472 &                0.598 &                     0.473 &                 0.609 &                     0.472 &                 0.613 \\
bowl        &                  0.358 &              0.368 &                    0.355 &                0.464 &                    0.355 &                0.454 &                     0.372 &                 0.492 &                     0.372 &                 0.492 &                    0.404 &                0.535 &                     0.403 &                 0.537 &                     0.405 &                 0.539 \\
bus         &                  0.446 &              0.472 &                    0.443 &                0.536 &                    0.434 &                0.522 &                     0.442 &                 0.542 &                     0.438 &                 0.534 &                    0.461 &                0.568 &                     0.466 &                 0.571 &                     0.465 &                 0.579 \\
cabinet     &                  0.372 &              0.396 &                    0.374 &                0.479 &                    0.371 &                0.469 &                     0.378 &                 0.489 &                     0.376 &                 0.486 &                    0.395 &                0.504 &                     0.393 &                 0.504 &                     0.396 &                 0.508 \\
camera      &                  0.376 &              0.399 &                    0.379 &                0.491 &                    0.377 &                0.486 &                     0.386 &                 0.503 &                     0.388 &                 0.504 &                    0.416 &                0.520 &                     0.419 &                 0.528 &                     0.415 &                 0.520 \\
can         &                  0.440 &              0.449 &                    0.420 &                0.525 &                    0.418 &                0.512 &                     0.407 &                 0.532 &                     0.407 &                 0.532 &                    0.410 &                0.547 &                     0.412 &                 0.551 &                     0.411 &                 0.552 \\
cap         &                  0.445 &              0.459 &                    0.448 &                0.535 &                    0.446 &                0.521 &                     0.460 &                 0.551 &                     0.455 &                 0.545 &                    0.476 &                0.589 &                     0.467 &                 0.585 &                     0.470 &                 0.590 \\
car         &                  0.366 &              0.386 &                    0.363 &                0.466 &                    0.361 &                0.457 &                     0.368 &                 0.478 &                     0.368 &                 0.474 &                    0.391 &                0.505 &                     0.395 &                 0.507 &                     0.394 &                 0.506 \\
cellphone   &                  0.439 &              0.507 &                    0.426 &                0.575 &                    0.418 &                0.562 &                     0.420 &                 0.570 &                     0.419 &                 0.564 &                    0.444 &                0.586 &                     0.444 &                 0.590 &                     0.440 &                 0.598 \\
chair       &                  0.468 &              0.497 &                    0.465 &                0.552 &                    0.461 &                0.543 &                     0.457 &                 0.559 &                     0.454 &                 0.555 &                    0.468 &                0.584 &                     0.467 &                 0.585 &                     0.466 &                 0.590 \\
clock       &                  0.400 &              0.425 &                    0.395 &                0.515 &                    0.391 &                0.508 &                     0.403 &                 0.530 &                     0.399 &                 0.524 &                    0.425 &                0.556 &                     0.420 &                 0.559 &                     0.421 &                 0.563 \\
dishwasher  &                  0.409 &              0.447 &                    0.408 &                0.515 &                    0.410 &                0.501 &                     0.420 &                 0.524 &                     0.416 &                 0.519 &                    0.437 &                0.527 &                     0.428 &                 0.527 &                     0.425 &                 0.531 \\
display     &                  0.424 &              0.459 &                    0.424 &                0.544 &                    0.417 &                0.535 &                     0.419 &                 0.553 &                     0.413 &                 0.547 &                    0.431 &                0.573 &                     0.435 &                 0.571 &                     0.435 &                 0.572 \\
earphone    &                  0.425 &              0.445 &                    0.415 &                0.540 &                    0.409 &                0.524 &                     0.414 &                 0.560 &                     0.415 &                 0.556 &                    0.459 &                0.581 &                     0.455 &                 0.582 &                     0.453 &                 0.589 \\
faucet      &                  0.536 &              0.565 &                    0.526 &                0.638 &                    0.522 &                0.630 &                     0.522 &                 0.657 &                     0.522 &                 0.653 &                    0.541 &                0.679 &                     0.542 &                 0.681 &                     0.554 &                 0.694 \\
file        &                  0.372 &              0.394 &                    0.376 &                0.473 &                    0.374 &                0.465 &                     0.380 &                 0.487 &                     0.377 &                 0.484 &                    0.399 &                0.503 &                     0.402 &                 0.501 &                     0.395 &                 0.508 \\
flowerpot   &                  0.382 &              0.395 &                    0.382 &                0.490 &                    0.382 &                0.483 &                     0.386 &                 0.509 &                     0.386 &                 0.506 &                    0.404 &                0.535 &                     0.404 &                 0.538 &                     0.405 &                 0.541 \\
guitar      &                  0.700 &              0.697 &                    0.655 &                0.756 &                    0.653 &                0.760 &                     0.628 &                 0.761 &                     0.617 &                 0.756 &                    0.601 &                0.745 &                     0.607 &                 0.761 &                     0.610 &                 0.776 \\
helmet      &                  0.348 &              0.357 &                    0.343 &                0.452 &                    0.341 &                0.444 &                     0.352 &                 0.479 &                     0.352 &                 0.478 &                    0.379 &                0.509 &                     0.383 &                 0.512 &                     0.379 &                 0.514 \\
jar         &                  0.408 &              0.422 &                    0.390 &                0.497 &                    0.389 &                0.488 &                     0.388 &                 0.512 &                     0.388 &                 0.510 &                    0.406 &                0.533 &                     0.404 &                 0.537 &                     0.404 &                 0.542 \\
keyboard    &                  0.522 &              0.551 &                    0.532 &                0.583 &                    0.523 &                0.573 &                     0.540 &                 0.596 &                     0.527 &                 0.610 &                    0.551 &                0.651 &                     0.555 &                 0.658 &                     0.566 &                 0.616 \\
knife       &                  0.808 &              0.819 &                    0.735 &                0.805 &                    0.740 &                0.798 &                     0.702 &                 0.796 &                     0.699 &                 0.790 &                    0.659 &                0.771 &                     0.671 &                 0.777 &                     0.661 &                 0.795 \\
lamp        &                  0.591 &              0.613 &                    0.556 &                0.663 &                    0.552 &                0.654 &                     0.541 &                 0.673 &                     0.539 &                 0.669 &                    0.536 &                0.679 &                     0.537 &                 0.686 &                     0.535 &                 0.691 \\
laptop      &                  0.502 &              0.512 &                    0.501 &                0.576 &                    0.496 &                0.557 &                     0.488 &                 0.573 &                     0.480 &                 0.568 &                    0.482 &                0.589 &                     0.479 &                 0.585 &                     0.487 &                 0.588 \\
loudspeaker &                  0.384 &              0.405 &                    0.386 &                0.492 &                    0.383 &                0.483 &                     0.390 &                 0.508 &                     0.389 &                 0.505 &                    0.406 &                0.527 &                     0.407 &                 0.529 &                     0.405 &                 0.531 \\
mailbox     &                  0.602 &              0.640 &                    0.593 &                0.688 &                    0.595 &                0.679 &                     0.585 &                 0.687 &                     0.586 &                 0.682 &                    0.557 &                0.677 &                     0.556 &                 0.682 &                     0.553 &                 0.695 \\
microphone  &                  0.603 &              0.631 &                    0.580 &                0.704 &                    0.571 &                0.702 &                     0.547 &                 0.715 &                     0.550 &                 0.697 &                    0.520 &                0.715 &                     0.529 &                 0.726 &                     0.525 &                 0.725 \\
microwaves  &                  0.398 &              0.413 &                    0.395 &                0.492 &                    0.393 &                0.478 &                     0.397 &                 0.510 &                     0.393 &                 0.507 &                    0.408 &                0.526 &                     0.409 &                 0.528 &                     0.410 &                 0.525 \\
motorbike   &                  0.412 &              0.435 &                    0.410 &                0.503 &                    0.404 &                0.499 &                     0.409 &                 0.519 &                     0.405 &                 0.515 &                    0.436 &                0.557 &                     0.447 &                 0.561 &                     0.448 &                 0.564 \\
mug         &                  0.334 &              0.343 &                    0.332 &                0.445 &                    0.331 &                0.438 &                     0.335 &                 0.465 &                     0.337 &                 0.463 &                    0.360 &                0.485 &                     0.366 &                 0.489 &                     0.363 &                 0.496 \\
piano       &                  0.418 &              0.441 &                    0.416 &                0.511 &                    0.412 &                0.501 &                     0.420 &                 0.523 &                     0.416 &                 0.519 &                    0.440 &                0.547 &                     0.443 &                 0.546 &                     0.449 &                 0.540 \\
pillow      &                  0.401 &              0.428 &                    0.397 &                0.510 &                    0.399 &                0.503 &                     0.411 &                 0.533 &                     0.410 &                 0.530 &                    0.440 &                0.570 &                     0.442 &                 0.572 &                     0.436 &                 0.572 \\
pistol      &                  0.532 &              0.560 &                    0.519 &                0.622 &                    0.511 &                0.613 &                     0.516 &                 0.624 &                     0.515 &                 0.611 &                    0.534 &                0.638 &                     0.540 &                 0.647 &                     0.523 &                 0.654 \\
printer     &                  0.405 &              0.416 &                    0.410 &                0.497 &                    0.408 &                0.488 &                     0.412 &                 0.509 &                     0.410 &                 0.506 &                    0.421 &                0.527 &                     0.427 &                 0.532 &                     0.419 &                 0.537 \\
remote      &                  0.497 &              0.540 &                    0.500 &                0.614 &                    0.487 &                0.605 &                     0.479 &                 0.601 &                     0.468 &                 0.591 &                    0.485 &                0.612 &                     0.480 &                 0.618 &                     0.485 &                 0.623 \\
rifle       &                  0.684 &              0.687 &                    0.654 &                0.745 &                    0.628 &                0.735 &                     0.619 &                 0.744 &                     0.618 &                 0.729 &                    0.612 &                0.748 &                     0.619 &                 0.757 &                     0.624 &                 0.760 \\
rocket      &                  0.681 &              0.702 &                    0.655 &                0.757 &                    0.603 &                0.740 &                     0.576 &                 0.738 &                     0.604 &                 0.714 &                    0.604 &                0.727 &                     0.602 &                 0.767 &                     0.605 &                 0.760 \\
skateboard  &                  0.580 &              0.617 &                    0.583 &                0.642 &                    0.577 &                0.624 &                     0.580 &                 0.636 &                     0.583 &                 0.639 &                    0.587 &                0.675 &                     0.595 &                 0.688 &                     0.588 &                 0.687 \\
sofa        &                  0.399 &              0.418 &                    0.402 &                0.495 &                    0.399 &                0.484 &                     0.404 &                 0.506 &                     0.402 &                 0.503 &                    0.420 &                0.532 &                     0.419 &                 0.534 &                     0.419 &                 0.534 \\
stove       &                  0.426 &              0.444 &                    0.424 &                0.521 &                    0.423 &                0.512 &                     0.427 &                 0.530 &                     0.426 &                 0.526 &                    0.435 &                0.539 &                     0.437 &                 0.541 &                     0.436 &                 0.545 \\
table       &                  0.449 &              0.467 &                    0.459 &                0.528 &                    0.455 &                0.519 &                     0.468 &                 0.547 &                     0.467 &                 0.544 &                    0.491 &                0.580 &                     0.490 &                 0.581 &                     0.491 &                 0.582 \\
telephone   &                  0.444 &              0.503 &                    0.422 &                0.577 &                    0.416 &                0.564 &                     0.416 &                 0.576 &                     0.414 &                 0.567 &                    0.438 &                0.594 &                     0.438 &                 0.601 &                     0.438 &                 0.607 \\
tower       &                  0.539 &              0.549 &                    0.516 &                0.612 &                    0.513 &                0.608 &                     0.498 &                 0.619 &                     0.497 &                 0.615 &                    0.486 &                0.627 &                     0.485 &                 0.636 &                     0.496 &                 0.642 \\
train       &                  0.465 &              0.499 &                    0.463 &                0.554 &                    0.453 &                0.543 &                     0.456 &                 0.565 &                     0.456 &                 0.557 &                    0.481 &                0.602 &                     0.486 &                 0.600 &                     0.485 &                 0.610 \\
trash       &                  0.359 &              0.370 &                    0.357 &                0.462 &                    0.357 &                0.455 &                     0.360 &                 0.474 &                     0.360 &                 0.473 &                    0.379 &                0.492 &                     0.381 &                 0.494 &                     0.381 &                 0.496 \\
washer      &                  0.380 &              0.411 &                    0.382 &                0.490 &                    0.382 &                0.480 &                     0.383 &                 0.502 &                     0.387 &                 0.502 &                    0.398 &                0.518 &                     0.393 &                 0.521 &                     0.393 &                 0.519 \\
watercraft  &                  0.561 &              0.590 &                    0.552 &                0.637 &                    0.542 &                0.625 &                     0.532 &                 0.637 &                     0.527 &                 0.623 &                    0.537 &                0.651 &                     0.535 &                 0.663 &                     0.533 &                 0.666 \\
\midrule
mean        &                  0.462 &              0.485 &                    0.455 &                0.555 &                    0.450 &                0.546 &                     0.451 &                 0.565 &                     0.450 &                 0.561 &                    0.464 &                0.585 &                     0.465 &                 0.589 &                     0.465 &                 0.592 \\
\bottomrule
\end{tabular}

==> tables/baseline_vs_best_cdl1.tex <==
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{3}{Model Name} & \multicolumn{2}{c}{No Augmentation} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.1} \\  
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
{} & Baseline & Ours & Baseline & Ours\\
% {} & Baseline (No augmentation) & Ours (No augmentation) & Baseline (R: 360, T: 0.1) & Ours (R: 360, T: 0.1) \\
% {} &                       CDL2 &                   CDL2 &                      CDL2 &                  CDL2 \\
% Model Name  &                            &                        &                           &                       \\
\midrule
airplane    &                      7.894 &                  7.789 &                    18.029 &                 8.078 \\
bag         &                     11.493 &                 10.147 &                    16.873 &                10.237 \\
basket      &                     13.827 &                 11.529 &                    17.710 &                11.683 \\
bathtub     &                     12.704 &                 11.019 &                    17.060 &                11.216 \\
bed         &                     13.275 &                 11.166 &                    17.393 &                11.518 \\
bench       &                      9.578 &                  8.700 &                    16.277 &                 8.872 \\
birdhouse   &                     15.461 &                 12.692 &                    18.789 &                12.857 \\
bookshelf   &                     13.430 &                 11.190 &                    17.512 &                11.332 \\
bottle      &                      9.734 &                  8.230 &                    11.854 &                 8.342 \\
bowl        &                     14.017 &                 11.876 &                    16.075 &                11.943 \\
bus         &                     10.633 &                  9.296 &                    15.508 &                 9.396 \\
cabinet     &                     12.762 &                 11.003 &                    17.467 &                10.991 \\
camera      &                     15.630 &                 13.105 &                    20.181 &                13.281 \\
can         &                     12.985 &                 10.708 &                    14.270 &                10.762 \\
cap         &                     11.646 &                 11.893 &                    18.423 &                11.763 \\
car         &                     13.587 &                 11.246 &                    18.298 &                11.451 \\
cellphone   &                      9.515 &                  8.294 &                    16.607 &                 8.454 \\
chair       &                     11.012 &                 10.002 &                    17.638 &                10.256 \\
clock       &                     12.431 &                 10.705 &                    19.336 &                10.754 \\
dishwasher  &                     12.902 &                 11.211 &                    18.047 &                11.244 \\
display     &                     11.120 &                  9.864 &                    17.992 &                10.128 \\
earphone    &                     13.484 &                 11.810 &                    19.407 &                12.231 \\
faucet      &                     10.810 &                 10.396 &                    17.695 &                10.952 \\
file        &                     13.224 &                 11.388 &                    17.588 &                11.472 \\
flowerpot   &                     15.277 &                 12.208 &                    17.507 &                12.403 \\
guitar      &                      5.615 &                  5.030 &                    11.997 &                 5.300 \\
helmet      &                     15.449 &                 13.345 &                    20.527 &                13.691 \\
jar         &                     13.707 &                 11.352 &                    15.783 &                11.452 \\
keyboard    &                      8.749 &                  7.686 &                    12.707 &                 8.224 \\
knife       &                      6.014 &                  5.070 &                    11.186 &                 5.424 \\
lamp        &                      9.868 &                  8.579 &                    13.346 &                 8.910 \\
laptop      &                      9.665 &                  8.666 &                    16.937 &                 8.998 \\
loudspeaker &                     14.025 &                 11.948 &                    18.819 &                12.072 \\
mailbox     &                      9.127 &                  8.075 &                    12.376 &                 8.180 \\
microphone  &                      9.907 &                  7.749 &                    14.480 &                 8.555 \\
microwaves  &                     13.666 &                 11.902 &                    17.712 &                11.917 \\
motorbike   &                     13.434 &                 10.647 &                    17.517 &                11.070 \\
mug         &                     15.523 &                 13.472 &                    18.008 &                13.429 \\
piano       &                     13.207 &                 11.633 &                    18.626 &                11.929 \\
pillow      &                     12.560 &                 10.525 &                    17.334 &                10.919 \\
pistol      &                      9.615 &                  8.494 &                    16.270 &                 8.998 \\
printer     &                     13.418 &                 11.935 &                    18.235 &                12.313 \\
remote      &                      9.500 &                  8.182 &                    15.390 &                 8.296 \\
rifle       &                      7.115 &                  6.324 &                    14.614 &                 6.605 \\
rocket      &                      6.796 &                  6.399 &                    13.363 &                 6.516 \\
skateboard  &                      8.234 &                  7.193 &                    12.328 &                 7.610 \\
sofa        &                     12.333 &                 10.754 &                    17.701 &                11.011 \\
stove       &                     12.745 &                 10.930 &                    16.854 &                11.073 \\
table       &                     10.546 &                  9.350 &                    14.353 &                 9.503 \\
telephone   &                      9.405 &                  8.224 &                    16.589 &                 8.374 \\
tower       &                     11.172 &                  8.877 &                    13.234 &                 9.081 \\
train       &                     10.769 &                  8.889 &                    15.503 &                 8.994 \\
trash       &                     14.985 &                 12.135 &                    16.791 &                12.176 \\
washer      &                     14.229 &                 12.291 &                    19.046 &                12.357 \\
watercraft  &                      9.362 &                  8.185 &                    14.358 &                 8.381 \\
\midrule
mean      &                     11.621 &                 10.024 &                    16.464 &                10.236 \\
\bottomrule
\end{tabular}

==> tables/baseline_vs_best_cdl2.tex <==
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{3}{Model Name} & \multicolumn{2}{c}{No Augmentation} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.1} \\  
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
{} & Baseline & Ours & Baseline & Ours\\
% {} & Baseline (No augmentation) & Ours (No augmentation) & Baseline (R: 360, T: 0.1) & Ours (R: 360, T: 0.1) \\
% {} &                       CDL2 &                   CDL2 &                      CDL2 &                  CDL2 \\
% Model Name  &                            &                        &                           &                       \\
\midrule
airplane    &                      0.269 &                  0.493 &                     6.275 &                 1.115 \\
bag         &                      0.527 &                  0.628 &                     3.656 &                 1.006 \\
basket      &                      0.726 &                  0.666 &                     2.573 &                 0.875 \\
bathtub     &                      0.643 &                  0.679 &                     2.983 &                 0.916 \\
bed         &                      0.758 &                  0.820 &                     3.887 &                 1.420 \\
bench       &                      0.381 &                  0.485 &                     4.699 &                 0.998 \\
birdhouse   &                      0.976 &                  1.003 &                     2.461 &                 1.249 \\
bookshelf   &                      0.712 &                  0.702 &                     3.157 &                 1.105 \\
bottle      &                      0.370 &                  0.363 &                     1.935 &                 0.751 \\
bowl        &                      0.679 &                  0.668 &                     1.736 &                 0.751 \\
bus         &                      0.422 &                  0.451 &                     3.123 &                 0.629 \\
cabinet     &                      0.553 &                  0.584 &                     2.421 &                 0.686 \\
camera      &                      1.095 &                  1.251 &                     4.156 &                 1.898 \\
can         &                      0.678 &                  0.557 &                     1.126 &                 0.582 \\
cap         &                      0.458 &                  0.951 &                     2.784 &                 1.213 \\
car         &                      0.636 &                  0.638 &                     3.583 &                 0.840 \\
cellphone   &                      0.321 &                  0.343 &                     3.518 &                 0.621 \\
chair       &                      0.492 &                  0.659 &                     4.493 &                 1.078 \\
clock       &                      0.620 &                  0.670 &                     3.703 &                 0.940 \\
dishwasher  &                      0.553 &                  0.583 &                     1.722 &                 0.596 \\
display     &                      0.476 &                  0.578 &                     3.706 &                 1.095 \\
earphone    &                      0.813 &                  1.007 &                     4.006 &                 1.796 \\
faucet      &                      0.710 &                  1.216 &                     5.347 &                 2.784 \\
file        &                      0.629 &                  0.685 &                     2.702 &                 0.959 \\
flowerpot   &                      1.012 &                  0.922 &                     2.495 &                 1.312 \\
guitar      &                      0.145 &                  0.175 &                     3.983 &                 1.412 \\
helmet      &                      0.988 &                  1.187 &                     3.284 &                 1.631 \\
jar         &                      0.772 &                  0.719 &                     2.160 &                 0.968 \\
keyboard    &                      0.297 &                  0.318 &                     4.304 &                 1.806 \\
knife       &                      0.195 &                  0.212 &                     4.020 &                 1.467 \\
lamp        &                      0.642 &                  0.741 &                     3.227 &                 1.589 \\
laptop      &                      0.319 &                  0.365 &                     4.809 &                 0.663 \\
loudspeaker &                      0.780 &                  0.832 &                     2.902 &                 1.130 \\
mailbox     &                      0.387 &                  0.545 &                     1.781 &                 0.819 \\
microphone  &                      0.697 &                  0.609 &                     4.229 &                 1.738 \\
microwaves  &                      0.669 &                  0.678 &                     1.999 &                 0.733 \\
motorbike   &                      0.751 &                  0.787 &                     4.191 &                 1.677 \\
mug         &                      0.907 &                  1.355 &                     2.286 &                 1.387 \\
piano       &                      0.764 &                  0.948 &                     3.812 &                 1.476 \\
pillow      &                      0.609 &                  0.588 &                     3.046 &                 0.856 \\
pistol      &                      0.431 &                  0.603 &                     5.601 &                 1.939 \\
printer     &                      0.734 &                  0.931 &                     3.646 &                 1.504 \\
remote      &                      0.358 &                  0.368 &                     4.259 &                 1.036 \\
rifle       &                      0.304 &                  0.371 &                     5.342 &                 1.033 \\
rocket      &                      0.226 &                  0.343 &                     3.998 &                 0.809 \\
skateboard  &                      0.280 &                  0.326 &                     4.194 &                 1.965 \\
sofa        &                      0.564 &                  0.638 &                     3.786 &                 1.023 \\
stove       &                      0.629 &                  0.679 &                     2.470 &                 1.109 \\
table       &                      0.465 &                  0.556 &                     3.275 &                 0.902 \\
telephone   &                      0.314 &                  0.341 &                     3.236 &                 0.588 \\
tower       &                      0.548 &                  0.495 &                     2.315 &                 1.207 \\
train       &                      0.503 &                  0.470 &                     3.500 &                 0.826 \\
trash       &                      0.796 &                  0.719 &                     1.602 &                 0.796 \\
washer      &                      0.745 &                  0.784 &                     2.067 &                 0.855 \\
watercraft  &                      0.413 &                  0.498 &                     4.277 &                 1.332 \\
\midrule
mean      &                      0.577 &                  0.651 &                     3.379 &                 1.154 \\
\bottomrule
\end{tabular}

==> tables/baseline_vs_best_fscore.tex <==
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{3}{Model Name} & \multicolumn{2}{c}{No Augmentation} & \multicolumn{2}{c}{R: $360^\circ$, T: 0.1} \\  
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
{} & Baseline & Ours & Baseline & Ours\\
% {} & Baseline (No augmentation) & Ours (No augmentation) & Baseline (R: 360, T: 0.1) & Ours (R: 360, T: 0.1) \\
% {} &                       CDL2 &                   CDL2 &                      CDL2 &                  CDL2 \\
% Model Name  &                            &                        &                           &                       \\
\midrule
airplane    &                      0.677 &                  0.648 &                     0.547 &                 0.646 \\
bag         &                      0.467 &                  0.521 &                     0.393 &                 0.522 \\
basket      &                      0.382 &                  0.472 &                     0.354 &                 0.471 \\
bathtub     &                      0.430 &                  0.492 &                     0.391 &                 0.491 \\
bed         &                      0.429 &                  0.501 &                     0.410 &                 0.501 \\
bench       &                      0.555 &                  0.574 &                     0.476 &                 0.573 \\
birdhouse   &                      0.380 &                  0.478 &                     0.360 &                 0.477 \\
bookshelf   &                      0.398 &                  0.479 &                     0.364 &                 0.479 \\
bottle      &                      0.549 &                  0.568 &                     0.483 &                 0.566 \\
bowl        &                      0.369 &                  0.465 &                     0.348 &                 0.464 \\
bus         &                      0.503 &                  0.522 &                     0.422 &                 0.524 \\
cabinet     &                      0.399 &                  0.468 &                     0.348 &                 0.469 \\
camera      &                      0.383 &                  0.478 &                     0.355 &                 0.479 \\
can         &                      0.405 &                  0.479 &                     0.365 &                 0.478 \\
cap         &                      0.427 &                  0.499 &                     0.385 &                 0.498 \\
car         &                      0.383 &                  0.461 &                     0.353 &                 0.460 \\
cellphone   &                      0.542 &                  0.550 &                     0.386 &                 0.549 \\
chair       &                      0.498 &                  0.537 &                     0.444 &                 0.537 \\
clock       &                      0.445 &                  0.505 &                     0.362 &                 0.505 \\
dishwasher  &                      0.390 &                  0.468 &                     0.337 &                 0.468 \\
display     &                      0.470 &                  0.513 &                     0.367 &                 0.513 \\
earphone    &                      0.449 &                  0.544 &                     0.412 &                 0.543 \\
faucet      &                      0.572 &                  0.641 &                     0.513 &                 0.640 \\
file        &                      0.395 &                  0.468 &                     0.349 &                 0.468 \\
flowerpot   &                      0.394 &                  0.490 &                     0.377 &                 0.489 \\
guitar      &                      0.875 &                  0.860 &                     0.703 &                 0.852 \\
helmet      &                      0.365 &                  0.465 &                     0.343 &                 0.465 \\
jar         &                      0.416 &                  0.492 &                     0.384 &                 0.492 \\
keyboard    &                      0.576 &                  0.576 &                     0.507 &                 0.573 \\
knife       &                      0.851 &                  0.860 &                     0.737 &                 0.854 \\
lamp        &                      0.640 &                  0.687 &                     0.573 &                 0.685 \\
laptop      &                      0.514 &                  0.533 &                     0.432 &                 0.533 \\
loudspeaker &                      0.400 &                  0.478 &                     0.357 &                 0.478 \\
mailbox     &                      0.636 &                  0.663 &                     0.564 &                 0.663 \\
microphone  &                      0.663 &                  0.733 &                     0.604 &                 0.729 \\
microwaves  &                      0.385 &                  0.466 &                     0.355 &                 0.466 \\
motorbike   &                      0.422 &                  0.503 &                     0.402 &                 0.503 \\
mug         &                      0.348 &                  0.449 &                     0.332 &                 0.449 \\
piano       &                      0.423 &                  0.493 &                     0.392 &                 0.492 \\
pillow      &                      0.425 &                  0.507 &                     0.385 &                 0.505 \\
pistol      &                      0.590 &                  0.620 &                     0.503 &                 0.619 \\
printer     &                      0.409 &                  0.484 &                     0.385 &                 0.483 \\
remote      &                      0.565 &                  0.576 &                     0.435 &                 0.575 \\
rifle       &                      0.780 &                  0.783 &                     0.658 &                 0.782 \\
rocket      &                      0.793 &                  0.788 &                     0.642 &                 0.791 \\
skateboard  &                      0.654 &                  0.646 &                     0.583 &                 0.645 \\
sofa        &                      0.435 &                  0.492 &                     0.395 &                 0.492 \\
stove       &                      0.427 &                  0.501 &                     0.386 &                 0.500 \\
table       &                      0.519 &                  0.546 &                     0.483 &                 0.545 \\
telephone   &                      0.548 &                  0.549 &                     0.381 &                 0.549 \\
tower       &                      0.549 &                  0.610 &                     0.507 &                 0.608 \\
train       &                      0.519 &                  0.550 &                     0.447 &                 0.552 \\
trash       &                      0.351 &                  0.450 &                     0.334 &                 0.450 \\
washer      &                      0.375 &                  0.458 &                     0.333 &                 0.458 \\
watercraft  &                      0.606 &                  0.627 &                     0.533 &                 0.627 \\
\midrule
mean      &                      0.497 &                  0.550 &                     0.436 &                 0.550 \\
\bottomrule
\end{tabular}
